SLOPE for Sparse Linear Regression:Asymptotics and Optimal Regularization

In sparse linear regression, the SLOPE estimator generalizes LASSO by penalizing different coordinates of the estimate according to their magnitudes. In this paper, we present a precise performance characterization of SLOPE in the asymptotic regime where the number of unknown parameters grows in proportion to the number of observations. Our asymptotic characterization enables us to derive the fundamental limits of SLOPE in both estimation and variable selection settings. We also provide a computational feasible way to optimally design the regularizing sequences such that the fundamental limits are reached. In both settings, we show that the optimal design problem can be formulated as certain infinite-dimensional convex optimization problems, which have efficient and accurate finite-dimensional approximations. Numerical simulations verify all our asymptotic predictions. They demonstrate the superiority of our optimal regularizing sequences over other designs used in the existing literature.

==> optimal_design.tex <==

\subsection{Proof of Proposition \ref{prop:function_space}\label{subsec:Proof-of-Proposition-functionspace}}

It directly follows from Proposition \ref{prop:prox} that $\Realizableset_{\mealim_{Y}}\subseteq\Lipndset$,
so we just need to show $\Lipndset\subseteq\Realizableset_{\mealim_{Y}}$.

For any $\proxfree\in\Lipndset$, consider the function $r(y)=y-\proxfree(y)$.
It can be easily verified that $r(y)\in\Lipndset$. We claim that
if we choose $\Lambda\sim r(|Y|)$ with $Y\sim\mealim_{Y}$, then
$\proxfree$ is the optimal solution of (\ref{eq:infinite_SLOPE})
(when $\tau=1$). Indeed, when $\tau=1$ and $\Lambda\sim r(|Y|)$,
(\ref{eq:infinite_SLOPE}) can be equivalently written as
\begin{align}
\text{Problem }\eqref{eq:infinite_SLOPE}\teq{\text{(a)}} & \min_{g\in\Lipndset}\frac{1}{2}\E_{\mu_{Y}}[|Y|-g(|Y|)]^{2}+\int_{0}^{1}F_{r(|Y|)}^{-1}(u)F_{g(|Y|)}^{-1}(u)du\nonumber \\
\teq{\text{(b)}} & \min_{g\in\Lipndset}\frac{1}{2}\E_{\mu_{Y}}[|Y|-g(|Y|)]^{2}+\E_{\mu_{Y}}[|Y|-\proxfree(|Y|)]g(|Y|)\nonumber \\
= & \min_{g\in\Lipndset}\frac{1}{2}\E_{\mu_{Y}}[\proxfree(|Y|)-g(|Y|)]^{2}+\frac{1}{2}\E_{\mu_{Y}}[Y^{2}-\proxfree^{2}(|Y|)],\label{eq:opti_lambda_problem_1}
\end{align}
where (a) follows from $g\in\Lipndset$ and in (b) we substitute $r(y)=y-\proxfree(y)$
and use the fact that $r\in\Lipndset$. From (\ref{eq:opti_lambda_problem_1}),
we can see $\proxfree$ is the optimal solution of (\ref{eq:infinite_SLOPE}).
On the other hand, since $f\in\Lipndset$ and $\E Y^{2}<\infty$,
we can verify that $\E\Lambda^{2}<\infty$ and hence $\Lambda\in\Wspace(\R)$.
In conclusion, for any $\proxfree\in\Lipndset$, we can always choose
$\Lambda\sim|Y|-\proxfree(|Y|)$ satisfying $\Lambda\in\Wspace(\R)$,
such that $\proxfree$ is the optimal solution of (\ref{eq:infinite_SLOPE})
(when $\tau=1$). By Proposition \ref{prop:prox}, this means $f(y)=\prox(y;\mealim_{Y},\mealim_{\Lambda})$
and hence $\proxfree\in\Realizableset_{\mealim_{Y}}$. Therefore,
$\Lipndset\subseteq\Realizableset_{\mealim_{Y}}$.

\subsection{Auxiliary Results for Proving Proposition \ref{prop:min_MSE}\label{subsec:Auxiliary-Results-for-estimation}}
\begin{lem}
\label{lem:f_sigma_unique_Lsigma_conti}For any $\sigma>0$, we have:
(I) optimization problem (\ref{eq:opt_esti_prox}) is convex and always
has a unique optimal solution $\proxfree_{\sigma}\in\Lipndset$, (II)
${\cal L}(\sigma)$ defined in (\ref{eq:opt_esti_prox}) is continuous
at $\sigma$.
\end{lem}
\begin{IEEEproof}
(I) Optimization problem (\ref{eq:opt_esti_prox}) can be equivalently
written as:
\[
\begin{aligned}\min_{\proxfree\in\Lipndset} & \E_{\mealim_{Y}}[\proxfree(Y)-\E(B\mid Y)]^{2}+\E_{\mealim_{Y}}[\text{Var}(B\mid Y)]\\
\st & \E_{\mealim_{Y}}\proxfree'(Y)\leq\delta.
\end{aligned}
\]
Then by the same arguments in the proof of Lemma \ref{lem:gstar_uniqueness},
it is not hard to check for any $\sigma>0$, it is (strongly) convex
and has a unique solution $\proxfree_{\sigma}\in\Lipndset$.

(II) Next, we prove the continuity of ${\cal L}(\sigma)$ at any $\sigma>0$.
Define the following set
\begin{equation}
\Lipndset_{\sigma}\bydef\{\proxfree\mid f\in\Lipndset\text{ and }\E\proxfree^{\prime}(B+\sigma H)\leq\delta\},\label{eq:set_Lipbd_sigma}
\end{equation}
where $H\sim\mathcal{N}(0,1)$ and $B\sim\mealim_{B}$ are independent.
Note that for any $\sigma>0$, we have $\Lipndset_{\sigma}\neq\emptyset$,
since $\{f=0\}\in\Lipndset_{\sigma}$.

The first step is to show for any $\sigma,r>0$, there exists $\veps\in(0,\sigma/2)$
such that whenever $\h{\sigma}\in\bdball_{\veps}(\sigma)$ and $\h{\proxfree}\in\Lipndset_{\hat{\sigma}}$,
we can always find a $\proxfree\in\Lipndset_{\sigma}$ satisfying
$|\proxfree(x)-\h{\proxfree}(x)|<r$ almost everywhere on $\R$. This
can be proved as follows. If $\h{\proxfree}\in\Lipndset_{\sigma}$,
we can choose $\proxfree=\h{\proxfree}$, which trivially satisfies
$|\proxfree(x)-\h{\proxfree}(x)|<r$; if $\h{\proxfree}\notin\Lipndset_{\sigma}$,
then $\E\h{\proxfree}'(B+\sigma H)>\delta$. Since $\hat{\proxfree}\in\Lipndset_{\hat{\sigma}}\subseteq\Lipndset$,
it follows that $|\h{\proxfree}'|\leq1$ almost everywhere on $\R$.
Meanwhile, since $\sigma,\h{\sigma}>0$, by the properties of Gaussian
convolution we know both $B+\hat{\sigma}H$ and $B+\sigma H$ have
smooth density functions supported on $\R$. Denote their density
functions as $q_{1}$ and $q_{2}$. Then we have 
\begin{align}
|\E\h{\proxfree}'(B+\h{\sigma}H)-\E\h{\proxfree}'(B+\sigma H)|= & \big|\int\h{\proxfree}'(y)[q_{1}(y)-q_{2}(y)]dy\big|\nonumber \\
\leq & \int|q_{1}(y)-q_{2}(y)|dy\nonumber \\
= & 2\text{TV}\big(\mealim_{B+\h{\sigma}H},\mealim_{B+\sigma H}\big)\nonumber \\
\tleq{\text{(a)}} & 2\text{TV}\big(\mealim_{\h{\sigma}H},\mealim_{\sigma H}\big)\nonumber \\
\tleq{\text{(b)}} & \sqrt{2\text{KL}(\mealim_{\h{\sigma}H},\mealim_{\sigma H})}\nonumber \\
\tleq{\text{(c)}} & C|\h{\sigma}-\sigma|,\label{eq:prox_hat_deri_diff_0}
\end{align}
where $\text{TV}(\cdot,\cdot)$ and $\text{KL}(\cdot,\cdot)$ denote
the total variation distance and KL-divergence between two probability
measures and $C>0$ is a fixed constant only depending on $\sigma$.
In reaching (\ref{eq:prox_hat_deri_diff_0}), (b) follows from Pinsker's
inequality and (c) follows from standard results of KL-divergence
between Gaussian random variables and the fact that $\veps\in(0,\sigma/2)$
and $\h{\sigma}\in\bdball_{\veps}(\sigma)$. Step (a) in (\ref{eq:prox_hat_deri_diff_0})
can be obtained as follows. Recall that $\Pi(\mealim_{1},\mealim_{2})$
denotes the set of all couplings between measures $\mealim_{1}$ and
$\mealim_{2}$. Then for any $(\h{\sigma}H_{1},\sigma H_{2})\in\Pi(\mealim_{\h{\sigma}H},\mealim_{\sigma H})$
and $B_{0}\sim\mealim_{B}$ independent of $(\h{\sigma}H_{1},\sigma H_{2})$,
we have $(B_{0}+\h{\sigma}H_{1},B_{0}+\sigma H_{2})\in\Pi(\mealim_{B+\h{\sigma}H},\mealim_{B+\sigma H})$.
Therefore, 
\begin{align}
\text{TV}\big(\mealim_{B+\h{\sigma}H},\mealim_{B+\sigma H}\big)\teq{\text{(a)}} & \inf_{\substack{(Y_{1},Y_{2})\in\Pi(\mealim_{B+\h{\sigma}H},\mealim_{B+\sigma H})}
}\P(Y_{1}\neq Y_{2})\nonumber \\
\leq & \inf_{\substack{(\h{\sigma}H_{1},\sigma H_{2})\in\Pi(\mealim_{\h{\sigma}H},\mealim_{\sigma H})\\
B_{0}\sim\mealim_{B}\text{ indep. of }(\h{\sigma}H_{1},\sigma H_{2})
}
}\P(B_{0}+\h{\sigma}H_{1}\neq B_{0}+\sigma H_{2})\nonumber \\
= & \inf_{\substack{(\h{\sigma}H_{1},\sigma H_{2})\in\Pi(\mealim_{\h{\sigma}H},\mealim_{\sigma H})}
}\P(\h{\sigma}H_{1}\neq\sigma H_{2})\nonumber \\
\teq{\text{(b)}} & \text{ TV}\big(\mealim_{\h{\sigma}H},\mealim_{\sigma H}\big),\label{eq:TV_bound_1}
\end{align}
where (a) and (b) follow from Strassen's Theorem \cite[p.7]{villani2003topics}.
From (\ref{eq:prox_hat_deri_diff_0}), when $\veps\in(0,\sigma/2)$
and $\h{\sigma}\in\bdball_{\veps}(\sigma)$,
\begin{equation}
\begin{aligned}|\E\h{\proxfree}'(B+\h{\sigma}H)-\E\h{\proxfree}'(B+\sigma H)| & \tleq{}C\veps.\end{aligned}
\label{eq:prox_hat_deri_diff}
\end{equation}
Since $\h{\proxfree}\in\Lipndset_{\hat{\sigma}}$, from (\ref{eq:set_Lipbd_sigma})
and (\ref{eq:prox_hat_deri_diff}) we get
\begin{equation}
\E\h{\proxfree}'(B+\sigma H)\leq\delta+C\veps.\label{eq:f_deri_aver_bd_1}
\end{equation}
We now slightly shrink $\h{\proxfree}$ to obtain the $\proxfree\in\Lipndset_{\sigma}$
satisfying $|\proxfree(x)-\h{\proxfree}(x)|<r$ almost everywhere.
On one hand, we know $B+\sigma H$ has a density function supported
on $\R$ for $\sigma>0$. On the other hand, since $\E\h{\proxfree}'(B+\sigma H)>\delta$
(due to $\h{\proxfree}\notin\Lipndset_{\sigma}$) and $|\h{\proxfree}'|\leq1$
almost everywhere, it is not hard to show if $\veps\leq\frac{\delta}{2C}$,
there exists some $\mathcal{A}\subset\R_{>0}$ such that $\E[\h{\proxfree}'(Y)\indicatorfn_{Y\in\mathcal{A}}]=C\veps$.
Accordingly, we set 
\[
\proxfree'(y)=\begin{cases}
0 & \pm y\in{\cal A},\\
\h{\proxfree}'(y) & \otherwise
\end{cases}
\]
and choose $\proxfree(y)$ to be:
\begin{equation}
\proxfree(y)=\int_{0}^{y}\proxfree'(t)dt.\label{eq:shrink_y_2}
\end{equation}
With this choice, from (\ref{eq:f_deri_aver_bd_1}) we have $\E f'(Y)\leq\delta-C\veps$
and thus $\proxfree\in\Lipndset_{\sigma}$. In addition, $0\leq\h{\proxfree}(x)-f(x)\leq2C\veps$
almost everywhere. Hence we can choose $\veps\leq\frac{r}{3C}$ so
that $0\leq\h{\proxfree}(x)-f(x)<r$ almost everywhere. Summing up,
for any $\sigma,r>0$, there exists $C$ depending only on $\sigma$
such that whenever $\veps\leq\min\{\frac{r}{3C},\tfrac{\sigma}{2}\}$,
$\h{\sigma}\in\bdball_{\veps}(\sigma)$ and $\h{\proxfree}\in\Lipndset_{\hat{\sigma}}$,
we can always find a $\proxfree\in\Lipndset_{\sigma}$ satisfying
$0\leq\h{\proxfree}(x)-f(x)<r$ almost everywhere on $\R$.

Define ${\cal L}(\proxfree,\sigma)\bydef\E[\proxfree(B+\varsigma H)-B]^{2}$,
which is the objective function in (\ref{eq:opt_esti_prox}). For
any compact interval $\minsigmaI\subseteq\R_{>0}$ and any $\sigma_{1},\sigma_{2}\in\minsigmaI$,
$\proxfree\in\Lipndset$, we have
\begin{align}
|\calL(\proxfree,\sigma_{1})-\calL(\proxfree,\sigma_{2})| & \leq\E\left|\proxfree^{2}(B+\sigma_{1}H)-\proxfree^{2}(B+\sigma_{2}H)\right|\nonumber \\
 & \quad+2\E|B||\proxfree(B+\sigma_{1}H)-\proxfree(B+\sigma_{2}H)|\nonumber \\
 & \leq\big(\sqrt{\E(|B+\sigma_{1}H|+|B+\sigma_{2}H|)^{2}}+2\sqrt{\E B^{2}}\big)|\sigma_{1}-\sigma_{2}|\nonumber \\
 & \leq C_{1}|\sigma_{1}-\sigma_{2}|,\label{eq:uniform_continuous_L}
\end{align}
where $C_{1}$ is a constant that only depends on $\minsigmaI$. Therefore,
for any $\proxfree\in\Lipndset$, $\calL(\proxfree,\sigma)$ is uniformly
Lipschitz continuous w.r.t. $\sigma$ on $\minsigmaI$. Consider $\proxfree_{\hat{\sigma}}$
which is the optimal solution of (\ref{eq:opt_esti_prox}) under $\hat{\sigma}$.
From the discussion in the last paragraph, for any $\sigma\in\minsigmaI$
and $r>0$, if $\h{\sigma}\in\bdball_{\veps}(\sigma)\bigcap\minsigmaI$
under small enough $\veps$, then there exists some $\proxfree\in\Lipndset_{\sigma}$
satisfying $|\proxfree_{\hat{\sigma}}(x)-f(x)|<r$ almost everywhere
on $\R$. Therefore, for this $\proxfree$ we have
\begin{equation}
\begin{aligned}|\calL(\proxfree_{\hat{\sigma}},\h{\sigma})-\calL(\proxfree,\sigma)| & \leq|\calL(\proxfree_{\hat{\sigma}},\h{\sigma})-\calL(\proxfree_{\hat{\sigma}},\sigma)|+|\calL(\proxfree_{\hat{\sigma}},\sigma)-\calL(\proxfree,\sigma)|\\
 & \leq C_{2}r,
\end{aligned}
\label{eq:L_f_sigma_perturbation}
\end{equation}
where $C_{2}$ is some constant that does not depend on $\veps,r$
and in the last step we use (\ref{eq:uniform_continuous_L}) and the
fact that $|\proxfree_{\hat{\sigma}}(x)-f(x)|<r$ almost everywhere.
Since $\calL(\h{\sigma})=\calL(\proxfree_{\hat{\sigma}},\h{\sigma})$,
we have from (\ref{eq:L_f_sigma_perturbation})
\begin{align*}
\calL(\h{\sigma}) & \tgeq{\text{(a)}}\calL(\proxfree,\sigma)-C_{2}r\tgeq{\text{(b)}}\calL(\sigma)-C_{2}r,
\end{align*}
where (a) follows from (\ref{eq:L_f_sigma_perturbation}) and (b)
follows from definition of $\calL(\sigma)$ in (\ref{eq:opt_esti_prox}).
By exchanging $\sigma$ and $\hat{\sigma}$, we can also get $\calL(\sigma)\geq\calL(\h{\sigma})-C_{2}r$.
In conclusion, for any compact interval $\minsigmaI\subseteq\R_{>0}$
and $r>0$, there exists $\veps>0$ such that for any $\sigma,\hat{\sigma}\in\minsigmaI$
satisfying $|\hat{\sigma}-\sigma|\leq\veps$, we have $|\calL(\h{\sigma})-\calL(\sigma)|\leq r$.
This proves the continuity of $\calL(\sigma)$ over $\R_{>0}$.
\end{IEEEproof}
%
\begin{lem}
\label{lem:min_sol_infA_lbd}Equation (\ref{eq:sigma_min_equation})
satisfies the following: (I) it always has a solution and the minimum
solution $\sigma_{0}\in[\sigma_{\noisei},(\sigma_{\noisei}^{2}+\delta^{-1}\E B^{2})^{1/2}]$,
(II) $\sigma_{0}=\inf\mathcal{A}$, where set $\mathcal{A}$ is defined
in (\ref{eq:sigmaset_def_1}).
\end{lem}
\begin{IEEEproof}
(I) We first prove $\sigma_{0}$ always exists and $\sigma_{0}\in\minsigmaI$,
where $\minsigmaI:=[\sigma_{\noisei},(\sigma_{\noisei}^{2}+\delta^{-1}\E B^{2})^{1/2}]$.
It is not hard to verify that at the boundary of $\minsigmaI$, ${\cal L}(\sigma)$
satisfies 
\begin{equation}
\begin{cases}
{\cal L}(\sigma)\leq\delta(\sigma^{2}-\sigma_{\noisei}^{2}) & \sigma=\big(\sigma_{\noisei}^{2}+\tfrac{\E B^{2}}{\delta}\big)^{1/2},\\
{\cal L}(\sigma)\geq\delta(\sigma^{2}-\sigma_{\noisei}^{2}) & \sigma=\sigma_{\noisei}.
\end{cases}\label{eq:L_sigma_bd_value}
\end{equation}
Indeed, when $\sigma=\big(\sigma_{\noisei}^{2}+\tfrac{\E B^{2}}{\delta}\big)^{1/2}$,
set $\proxfree=0$ in (\ref{eq:opt_esti_prox}) and $\E[\proxfree(B+\sigma H)-B]^{2}=\E B^{2}=\delta(\sigma^{2}-\sigma_{\noisei}^{2})$,
so ${\cal L}(\sigma)\leq\delta(\sigma^{2}-\sigma_{\noisei}^{2})$.
On the other hand, since ${\cal L}(\sigma)\geq0$, the second inequality
of (\ref{eq:L_sigma_bd_value}) immediately follows. Then by (\ref{eq:L_sigma_bd_value}),
the continuity of ${\cal L}(\sigma)$ shown in Lemma \ref{lem:f_sigma_unique_Lsigma_conti}
and the fact that $\sigma_{0}\geq\sigma_{\noisei}$, we know $\sigma_{0}$
always exists and $\sigma_{0}\in\minsigmaI$.

(II) To prove $\inf\mathcal{A}=\sigma_{0}$, we proceed as follows:
\begin{enumerate}
\item[(i)] Show
\begin{equation}
\inf\mathcal{A}\in\minsigmaI.\label{eq:inf_A_bounded}
\end{equation}
\item[(ii)] Prove the following membership certificate of set $\mathcal{A}$
for those $\sigma\in\minsigmaI$:
\begin{equation}
\sigma\in\mathcal{A}\Longleftrightarrow{\cal L}(\sigma)\leq\delta(\sigma^{2}-\sigma_{\noisei}^{2}).\label{eq:membership_cert}
\end{equation}
\end{enumerate}
It is not hard to see the above steps will imply $\inf\mathcal{A}=\sigma_{0}$.
Indeed, combining (\ref{eq:membership_cert}) with (\ref{eq:inf_A_bounded})
yields the following characterization of $\inf\mathcal{A}$: 
\begin{equation}
\inf\mathcal{A}=\inf\big\{\sigma\mid\sigma\in\minsigmaI\text{ and }{\cal L}(\sigma)\leq\delta(\sigma^{2}-\sigma_{\noisei}^{2})\big\}.\label{eq:char_inf_A}
\end{equation}
By (\ref{eq:L_sigma_bd_value}) and the continuity of ${\cal L}(\sigma)$,
the infimum on the RHS of (\ref{eq:char_inf_A}) is reached by $\sigma_{0}$,
which always exists. Therefore, $\inf\mathcal{A}=\sigma_{0}$. Step
(i)-(ii) can be proved as follows:

{[}Proof of (i){]} From the first equation of (\ref{eq:sigma2_cond1}),
we have $\inf\mathcal{A}\geq\sigma_{\noisei}$. On the other hand,
since $\proxfree=0$, $\sigma=\big(\sigma_{\noisei}^{2}+\tfrac{\E B^{2}}{\delta}\big)^{1/2}$,
$\tau=1$ is a solution of (\ref{eq:fixed_point_equation_f_sigmatau_1})-(\ref{eq:fixed_point_equation_f_sigmatau_2}),
from (\ref{eq:sigopt_2}) we have $\optsig\leq\big(\sigma_{\noisei}^{2}+\tfrac{\E B^{2}}{\delta}\big)^{1/2}$.
This together with the lower bound of $\optsig$ in (\ref{eq:sig_opt_lbd_1})
indicates: $\inf\mathcal{A}\leq\optsig\leq\big(\sigma_{\noisei}^{2}+\tfrac{\E B^{2}}{\delta}\big)^{1/2}$.
Therefore, $\inf\mathcal{A}\in\minsigmaI$.

{[}Proof of (ii){]} The ``$\Rightarrow$'' direction of (\ref{eq:membership_cert})
immediately follows from the definition of $\mathcal{A}$ in (\ref{eq:sigmaset_def_1}).
For the other direction, suppose we have a $\sigma\in\minsigmaI$
satisfying ${\cal L}(\sigma)\leq\delta(\sigma^{2}-\sigma_{\noisei}^{2})$.
Then 
\begin{equation}
\E[\proxfree_{\sigma}(B+\sigma H)-B]^{2}={\cal L}(\sigma)\leq\delta(\sigma^{2}-\sigma_{\noisei}^{2}),\label{eq:onepoint_small}
\end{equation}
where the first equality is due to that ${\cal L}(\sigma)$ can be
achieved by $\proxfree_{\sigma}$. Now consider the shrinkage of $\proxfree_{\sigma}$
as: $\alpha\proxfree_{\sigma}$, where $\alpha\in[0,1]$. Clearly,
for any $\alpha\in[0,1]$, $\alpha\proxfree_{\sigma}$ still satisfies
$\E[\alpha\proxfree_{\sigma}'(B+\sigma H)]\leq\delta$. Also we have:
\begin{equation}
\E[0\cdot\proxfree_{\sigma}(B+\sigma H)-B]^{2}=\E B^{2}\geq\delta(\sigma^{2}-\sigma_{\noisei}^{2}),\label{eq:zeropoint_large}
\end{equation}
where the last inequality follows from the condition that $\sigma\in\minsigmaI$.
On the other hand, it can be easily checked that $\alpha\mapsto\E[\alpha\proxfree_{\sigma}(B+\sigma H)-B]^{2}$
is continuous, so from (\ref{eq:zeropoint_large}), (\ref{eq:onepoint_small}),
there exists $\alpha_{0}\in[0,1]$ such that $(\alpha_{0}\proxfree_{\sigma},\sigma)$
is a solution of (\ref{eq:sigma2_cond1}), indicating $\sigma\in\mathcal{A}$.
\end{IEEEproof}

\subsection{Auxiliary Results for Proving Proposition \ref{prop:max_power}\label{subsec:Auxiliary-Results-for-testing}}
\begin{lem}
\label{lem:function_space1}For a probability measure $\mealim_{Y}\in\Wspace(\R)$,
define
\begin{equation}
\begin{aligned}\widetilde{\mathcal{M}}_{\mealim_{Y}}\bydef\big\{\prox(\cdot\,;\mealim_{Y},\mealim_{\Lambda}) & \mid\mealim_{\Lambda}\in\Wspace(\R)\text{ and }\text{if }\probthreshzero>0,\\
 & {\textstyle \int_{t}^{\probthreshzero}F_{\Lambda}^{-1}(u)du>\int_{t}^{\probthreshzero}F_{|Y|}^{-1}(u)du,\forall t\in[0,\probthreshzero)\big\}}
\end{aligned}
\label{eq:feasible_denoiser_2}
\end{equation}
where $\probthreshzero=\P\big(\prox(Y;\mealim_{Y},\mealim_{\Lambda})=0\big)$.
Then for any $\mealim_{Y}\in\Wspace(\R)$, we have $\widetilde{\mathcal{M}}_{\mealim_{Y}}=\Lipndset$.
Correspondingly, for any $\proxfree(y)\in\Lipndset$ and $\ythreshzero=\sup_{y\geq0}\left\{ y\mid\proxfree(y)=0\right\} $,
we can take $\Lambda\sim\max\{\ythreshzero,|Y|-\proxfree(|Y|)\}$,
with $Y\sim\mealim_{Y}$, so that $\prox(y\,;\mealim_{Y},\mealim_{\Lambda})=\proxfree(y)$.
\end{lem}
\begin{IEEEproof}
The proof is similar as Proposition \ref{prop:function_space}. When
$\Lambda\sim\max\{\ythreshzero,|Y|-\proxfree(|Y|)\}$, optimization
(\ref{eq:infinite_SLOPE}) becomes:
\begin{equation}
\begin{aligned} & \min_{g\in\Lipndset}\frac{1}{2}\E\big\{[\proxfree(|Y|)-g(|Y|)]^{2}\indicatorfn_{|Y|\geq\ythreshzero}\big\}+\frac{1}{2}\E\big\{[(|Y|-\ythreshzero)-g(|Y|)]^{2}\indicatorfn_{|Y|<\ythreshzero}\big\}\\
 & \qquad+\frac{1}{2}\E Y^{2}-\E[|Y|-f(|Y|)]^{2}.
\end{aligned}
\label{eq:opti_lambda_problem_2}
\end{equation}
Since the feasible set in (\ref{eq:opti_lambda_problem_2}) is $\Lipndset$,
the optimal solution of (\ref{eq:opti_lambda_problem_2}) equals to
$\proxfree$. Recall that $\prox(y;\mealim_{Y},\mealim_{\Lambda})$
is the optimal solution of (\ref{eq:infinite_SLOPE}), so we have
$\prox(y;\mealim_{Y},\mealim_{\Lambda})=\proxfree(y)$.

Finally, we show $\Lambda\sim\max\{\ythreshzero,|Y|-\proxfree(|Y|)\}$
satisfies the constraint in (\ref{eq:feasible_denoiser_2}). Since
$\mealim_{Y}\in\Wspace(\R)$ and $\Lambda\leq|Y|-\proxfree(|Y|)\leq|Y|$,
we can easily get $\mealim_{\Lambda}\in\Wspace(\R)$. On the other
hand, suppose $\probthreshzero>0$. For any $t\in[0,\probthreshzero)$,
we have
\[
\begin{aligned}\int_{t}^{\probthreshzero}F_{|Y|}^{-1}(u)du & \teq{\text{(a)}}\E\big(\indicatorfn_{F_{|Y|}^{-1}(t)\leq|Y|\leq\ythreshzero}\cdot|Y|\big)\\
 & \tle{\text{(b)}}\ythreshzero\P\big(F_{|Y|}^{-1}(t)\leq|Y|\leq\ythreshzero\big)\\
 & =\ythreshzero(\probthreshzero-t)\\
 & \teq{\text{(c)}}\int_{t}^{\probthreshzero}F_{\Lambda}^{-1}(u)du,
\end{aligned}
\]
where in (a) we use the fact that $F_{|Y|}^{-1}(\probthreshzero)=\ythreshzero$,
since $\prox(y;\mealim_{Y},\mealim_{\Lambda})=\proxfree(y)$, (b)
follows from $F_{|Y|}^{-1}(t)<F_{|Y|}^{-1}(\probthreshzero)=\ythreshzero$
and (c) is due to our choice of $\Lambda$, which yields $F_{\Lambda}^{-1}(u)=\ythreshzero$
for any $0\leq u\leq\probthreshzero$.
\end{IEEEproof}
\begin{lem}
\label{lem:f_sigma_unique_L_alpha_sigma_conti}For $\alpha\in[0,1]$
and $\sigma>0$, we have: (I) optimization problem (\ref{eq:opt_testing_prox})
is convex and always has a unique optimal solution $\proxfree_{\alpha,\sigma}\in\Lipndset$,
(II) $\mathcal{L}_{\alpha}(\sigma)$ defined in (\ref{eq:opt_testing_prox})
is a continuous function over $\R_{>0}$, (III) equation $\mathcal{L}_{\alpha}(\sigma)=\delta(\sigma^{2}-\sigma_{\noisei}^{2})$
always has a solution and the minimum solution $\tminsigsol\in\big[\sigma_{\noisei},\,\sqrt{\sigma_{\noisei}^{2}+\delta^{-1}\E B^{2}}\big]$.
\end{lem}
\begin{IEEEproof}
(I) Comparing with (\ref{eq:opt_esti_prox}) and (\ref{eq:opt_testing_prox}),
we can find the only difference is that in (\ref{eq:opt_testing_prox}),
we add a constraint $\proxfree\in\softfunset$. It is not hard to
check for any $\alpha\in[0,1]$ and $\sigma>0$, the set $\softfunset$
is convex and closed in the $L^{2}$ space $\Lyspace_{\mu_{Y}}$ {[}definition
can be found in (\ref{eq:L2space_mealim_Y}){]}, so the uniqueness
of optimal solution of (\ref{eq:opt_testing_prox}) still holds using
the same arguments.

(II) The case of $\alpha=0\text{ or }1$ is easy. When $\alpha=1$,
we have $\Lipndset\subseteq\softfunset$, so $\mathcal{L}_{\alpha}(\sigma)=\mathcal{L}(\sigma)$
and its continuity is proved in the last part of Lemma \ref{lem:f_sigma_unique_Lsigma_conti};
when $\alpha=0$, $\softfunset$ contains only one element: $\proxfree(x)=0$
and $\mathcal{L}_{\alpha}(\sigma)=\E B^{2}$, which is trivially continuous.
Therefore, it only remains to verify for the case when $\alpha\in(0,1)$.

The proof for case $\alpha\in(0,1)$ is similar to the proof of continuity
of $\mathcal{L}(\sigma)$ in Lemma \ref{lem:f_sigma_unique_Lsigma_conti}.
For any $\alpha\in(0,1)$ and $\sigma>0$, define the following set
\begin{equation}
\Lipndset_{\alpha,\sigma}\bydef\{\proxfree\mid f\in\Lipndset\cap\softfunset\text{ and }\E\proxfree^{\prime}(B+\sigma H)\leq\delta\},\label{eq:set_Lipbd_sigma-1}
\end{equation}
where $H\sim\mathcal{N}(0,1)$ and $B\sim\mealim_{B}$ are independent.
We always have $\Lipndset_{\alpha,\sigma}\neq\emptyset$, since $\{f=0\}\in\Lipndset_{\alpha,\sigma}$.
Next we show that for any $\alpha\in(0,1)$ and $\sigma,r>0$, there
exists $\veps\in(0,\sigma/2)$ such that whenever $\h{\sigma}\in\bdball_{\veps}(\sigma)$
and $\h{\proxfree}\in\Lipndset_{\alpha,\hat{\sigma}}$, we can always
find a $\proxfree\in\Lipndset_{\alpha,\sigma}$ satisfying $|\proxfree(x)-\h{\proxfree}(x)|<r$
almost everywhere on $\R$. First, for any $\hat{\sigma}>0$ and $\h{\proxfree}\in\Lipndset_{\alpha,\hat{\sigma}}$,
we have $|\h{\proxfree}(y)|=0$, when $|y|\leq\Phi^{-1}(1-\tfrac{\alpha}{2})\hat{\sigma}$.
We can then apply the following shrinkage to $\h{\proxfree}$:
\begin{equation}
\h{\proxfree}_{T}(y)=\sgn(y)\max\{0,\h{\proxfree}(|y|)-\Phi^{-1}(1-\tfrac{\alpha}{2})|\sigma-\hat{\sigma}|\}.\label{eq:f_shrunk_1}
\end{equation}
One can check $\h{\proxfree}_{T}$ in (\ref{eq:f_shrunk_1}) satisfies:
$\h{\proxfree}_{T}\in\Lipndset_{\alpha,\hat{\sigma}}\cap\softfunset$
and 
\begin{equation}
0\leq\hat{\proxfree}(y)-\h{\proxfree}_{T}(y)\leq\Phi^{-1}(1-\tfrac{\alpha}{2})|\sigma-\hat{\sigma}|\label{eq:fhat_fT_diff}
\end{equation}
almost everywhere on $\R$. For small enough $\veps>0$ and $\h{\sigma}\in\bdball_{\veps}(\sigma)$,
we can then follow the same steps leading to (\ref{eq:shrink_y_2})
in the proof of continuity of $\mathcal{L}(\sigma)$ in Lemma \ref{lem:f_sigma_unique_Lsigma_conti}
to obtain a $\proxfree\in\Lipndset$ satisfying 
\begin{equation}
0\leq\h{\proxfree}_{T}(y)-\proxfree(y)\leq\frac{r}{2}\label{eq:fT_f_diff}
\end{equation}
almost everywhere on $\R$ and $\E\proxfree^{\prime}(B+\sigma H)\leq\delta$.
Meanwhile, since $\h{\proxfree}_{T}\in\softfunset$, we also have
$\proxfree\in\softfunset$. As a result, $\proxfree\in\Lipndset_{\alpha,\sigma}$.
Besides, combining (\ref{eq:fhat_fT_diff}) and (\ref{eq:fT_f_diff})
we have for small enough $\veps>0$ and $\h{\sigma}\in\bdball_{\veps}(\sigma)$,
$0\leq\hat{\proxfree}(y)-\proxfree(y)\leq r$ almost everywhere on
$\R$. The remaining proof is completely same as the last part of
the proof of $\mathcal{L}(\sigma)$'s continuity and we omit the details
here.

(III) The proof is the same as Lemma \ref{lem:min_sol_infA_lbd}.
Using the same argument, it can be verified that $\mathcal{L}_{\alpha}(\sigma)$
also satisfies 
\[
\begin{cases}
\mathcal{L}_{\alpha}(\sigma)\leq\delta(\sigma^{2}-\sigma_{\noisei}^{2}) & \sigma=\big(\sigma_{\noisei}^{2}+\tfrac{\E B^{2}}{\delta}\big)^{1/2},\\
\mathcal{L}_{\alpha}(\sigma)\geq\delta(\sigma^{2}-\sigma_{\noisei}^{2}) & \sigma=\sigma_{\noisei}.
\end{cases}
\]
Then by the continuity of $\mathcal{L}_{\alpha}(\sigma)$ and the
fact that $\tminsigsol\geq\sigma_{\noisei}$, we get the desired result.
\end{IEEEproof}
\begin{lem}
\label{lem:testing_tightness_cond_1}For any given $\alpha\in[0,1]$,
we have
\begin{enumerate}
\item[(a)] It is always true that $\optsig(\alpha)\geq\tminsigsol$.
\item[(b)]  If $\delta^{-1}\E\big[\proxfree_{\alpha}'(\toptY)\big]<1$, then
$\optsig(\alpha)=\tminsigsol$ and the infimum of (\ref{eq:slope_test_opt_ubd1})
can be achieved by choosing $\mealim_{\Lambda}=\mealim_{\text{opt},\alpha}$.
\end{enumerate}
\end{lem}
\begin{IEEEproof}
The proof is similar to that of Proposition \ref{prop:min_MSE} (c).
Recall that a key step in the proof is the conversion of the optimization
over $\mealim_{\Lambda}$ into an equivalent optimization over realizable
limiting scalar functions $\proxfree$. We want to adopt the same
strategy here, but since an additional constraint on $\mealim_{\Lambda}$
is added, we need to determine the new realizable set of $\proxfree$,
as we did in Proposition \ref{prop:function_space}. It turns out
that the new realizable set is still $\Lipndset$. This result is
proved in In Lemma \ref{lem:function_space1} and it enables us to
follow the same steps leading to (\ref{eq:sigopt_2}) to show that
(\ref{eq:slope_test_opt_ubd1}) is equivalent to
\begin{equation}
\begin{aligned}\optsig(\alpha)= & \inf\{\sigma\mid(\sigma,\tau)\in\mathcal{D}_{F}(\alpha),\text{ for some }\text{\ensuremath{\tau>0}}\},\end{aligned}
\label{eq:slope_test_opt_ubd2}
\end{equation}
where $\mathcal{D}_{F}(\alpha)$ is defined as:
\[
\mathcal{D}_{F}(\alpha)\bydef\big\{(\sigma,\tau)\in\R_{>0}^{2}:\,\exists\proxfree\in\Lipndset\cap\softfunset\text{ s.t. }(\proxfree,\sigma,\tau)\text{ satisfies \eqref{eq:fixed_point_equation_f_sigmatau_1}-\eqref{eq:fixed_point_equation_f_sigmatau_2}}\big\}.
\]
\begin{comment}
with $\softfunset\bydef\big\{\proxfree(y):\proxfree(y)=0\text{ for }|y|\leq\Phi^{-1}(1-\tfrac{\alpha}{2})\sigma\big\}$.
\end{comment}
Comparing (\ref{eq:sigopt_2}) and (\ref{eq:slope_test_opt_ubd2}),
it can be seen that the only difference is that in (\ref{eq:slope_test_opt_ubd2})
we require $f\in\softfunset$, which is needed to control the type-I
error level. Then similar as (\ref{eq:sigmaset_def_1}) we define
\[
\mathcal{A}(\alpha)\bydef\big\{\sigma\in\R_{>0}:\,\exists\proxfree\in\Lipndset\cap\softfunset,\text{s.t. \ensuremath{(\proxfree,\sigma)}\text{ satisfies \eqref{eq:sigma2_cond1}}}\big\}
\]
and it holds that $\optsig(\alpha)\geq\inf\mathcal{A}(\alpha)$. Meanwhile,
by the same reasoning in Lemma \ref{lem:min_sol_infA_lbd}, we can
also show $\inf\mathcal{A}(\alpha)=\tminsigsol$. This gives us $\optsig(\alpha)\geq\tminsigsol$.

Now consider the scenario where $\delta^{-1}\E\big[\proxfree_{\alpha}'(\toptY)\big]<1$.
In this case, we have $\tmintausol\in(0,\infty)$. Then it is not
hard to check $(\proxfree_{\alpha},\tminsigsol,\tmintausol)$ satisfies
equation (\ref{eq:fixed_point_equation_f_sigmatau_1})-(\ref{eq:fixed_point_equation_f_sigmatau_2}).
Therefore, $(\tminsigsol,\tmintausol)\in\mathcal{D}_{F}(\alpha)$.
By (\ref{eq:slope_test_opt_ubd2}), we have $\tminsigsol\geq\optsig(\alpha)$.
Since we already get $\optsig(\alpha)\geq\tminsigsol$, we can conclude
that $\optsig(\alpha)=\tminsigsol$. Let us denote $(\sigOpt,\tauOpt)$
as the solution of fixed-point equation (\ref{eq:sigmatau_1})-(\ref{eq:sigmatau_2}),
when $\mealim_{\Lambda}=\mealim_{\text{opt},\alpha}$. Using Lemma
\ref{lem:function_space1}, it is not hard to check 
\begin{equation}
(\sigOpt,\tauOpt)=(\tminsigsol,\tmintausol)\label{eq:sigmastar_reached}
\end{equation}
and 
\begin{equation}
\prox(y;\mealim_{\YOpt},\mealim_{\tauOpt\Lambda})=\proxfree_{\alpha}(y).\label{eq:falpha_y_reached}
\end{equation}
Meanwhile, we have $\mealim_{\text{opt},\alpha}\in\tLamspace$. Recall
that the infimum of $\sigOpt$ in (\ref{eq:slope_test_opt_ubd1})
is $\tminsigsol$ {[}c.f. (\ref{eq:slope_test_opt_ubd2}){]}. As a
result, the infimum of $\sigOpt$ in (\ref{eq:slope_test_opt_ubd1})
is reached when $\mealim_{\Lambda}=\mealim_{\text{opt},\alpha}$.
\end{IEEEproof}
\begin{lem}
\label{lem:testing_tightness_cond_2}For $\alpha\in(0,1]$, if $\delta^{-1}\E\big[\proxfree_{\alpha}'(\toptY)\big]<1$,
then $\overline{\mathcal{\limpower}}(\alpha)=\limpower(\alpha)$ and
the equality is attained when $\mealim_{\Lambda}=\mealim_{\text{opt},\alpha}$.
\end{lem}
\begin{IEEEproof}
By Lemma \ref{lem:testing_tightness_cond_1} and (\ref{eq:power_ubd2}),
we know it suffices to show $\limpower(\alpha)=\overline{\mathcal{\limpower}}(\alpha)$,
since when $\delta^{-1}\E\big[\proxfree_{\alpha}'(\toptY)\big]<1$,
we have $\optsig(\alpha)=\tminsigsol$.

We first prove the result: if $\delta^{-1}\E\big[\proxfree_{\alpha}'(\toptY)\big]<1$
and $\tythreshzero=\Phi^{-1}(1-\frac{\alpha}{2})\tminsigsol$, then
$\overline{\mathcal{\limpower}}(\alpha)=\limpower(\alpha)$. This
can be done as follows. Assume $\delta^{-1}\E\big[\proxfree_{\alpha}'(\toptY)\big]<1$
and $\tythreshzero=\Phi^{-1}(1-\frac{\alpha}{2})\tminsigsol$. In
the remaining proof, let $(\sigOpt,\tauOpt)$ be the solution of fixed-point
equation (\ref{eq:sigmatau_1})-(\ref{eq:sigmatau_2}), when $\mealim_{\Lambda}=\mealim_{\text{opt},\alpha}$
and $\ythresh=\sup_{y\geq0}\{y\mid\prox(y;\mealim_{\YOpt},\mealim_{\tauOpt\Lambda})=0\}$.
Recall from the proof of Lemma \ref{lem:testing_tightness_cond_1},
we know when $\mealim_{\Lambda}=\mealim_{\text{opt},\alpha}$, we
have
\[
\ythresh\teq{\text{(a)}}\tythreshzero\teq{\text{(b)}}\Phi^{-1}(1-\frac{\alpha}{2})\tminsigsol\teq{\text{(c)}}\Phi^{-1}(1-\frac{\alpha}{2})\sigOpt,
\]
where (a) follows from (\ref{eq:falpha_y_reached}), (b) follows from
assumption $\tythreshzero=\Phi^{-1}(1-\frac{\alpha}{2})\tminsigsol$
and (c) from (\ref{eq:sigmastar_reached}). Therefore, 
\begin{align}
\P(|B+\sigOpt H|\geq\ythresh\mid B\neq0) & =\P\big(|B+\sigOpt H|\geq\Phi^{-1}(1-\tfrac{\alpha}{2})\sigOpt\mid B\neq0\big)\nonumber \\
 & =\overline{\mathcal{\limpower}}(\alpha),\label{eq:P_ubd_tight_2}
\end{align}
where the last equality is due to that $\mealim_{\text{opt},\alpha}$
is the optimal solution of (\ref{eq:slope_test_opt_ubd1}), as is
proved by Lemma \ref{lem:testing_tightness_cond_1}. Therefore, from
(\ref{eq:P_ubd_tight_2}) we know when $\mealim_{\Lambda}=\mealim_{\text{opt},\alpha}$,
the objective value of (\ref{eq:slope_test_opt}) equals to $\overline{\mathcal{\limpower}}(\alpha)$.
This implies $\limpower(\alpha)\geq\overline{\mathcal{\limpower}}(\alpha)$,
since $\limpower(\alpha)$ is the optimal value of (\ref{eq:slope_test_opt}).
Combined with the fact that $\overline{\mathcal{\limpower}}(\alpha)$
is the upper bound of $\limpower(\alpha)$ {[}c.f. (\ref{eq:power_ubd2}){]},
it then follows that $\overline{\mathcal{\limpower}}(\alpha)=\limpower(\alpha)$.

We now prove $\limpower(\alpha)=\overline{\mathcal{\limpower}}(\alpha)$
by contradiction. Suppose under the Type-I error level $\alpha$,
$\limpower(\alpha)<\overline{\mathcal{\limpower}}(\alpha)$. Then
by the claim above, we must have $y_{0}(\alpha)>\Phi^{-1}(1-\frac{\alpha}{2})\sigma_{0}(\alpha)$.%
\begin{comment}
Also the infimum at (\ref{eq:slope_test_opt_ubd1}) can be attained
by choosing $\mealim_{\Lambda}=\mealim_{\text{opt},\alpha}$.
\end{comment}
\begin{comment}
In the remaining proof, $(\sigOpt,\tauOpt)$ will be used to denote
the solution of (\ref{eq:sigmatau_1})-(\ref{eq:sigmatau_2}) when
$\mealim_{\Lambda}=\mealim_{\text{opt},\alpha}$ and $\ythresh$ will
be used to denote the corresponding zero threshold of $\prox$: $\sup_{y\geq0}\{y\mid\prox(y;\mealim_{\YOpt},\mealim_{\tauOpt\Lambda})=0\}$.
\end{comment}
Recall that $\sigOpt=\sigma_{0}(\alpha)$ and $\ythresh=y_{0}(\alpha)$,
so we get
\[
\ythresh=y_{0}(\alpha)>\Phi^{-1}(1-\frac{\alpha}{2})\sigma_{0}(\alpha)=\Phi^{-1}(1-\frac{\alpha}{2})\sigOpt
\]
or equivalently, $\P(|\sigOpt H|\geq\ythresh)<\alpha$. This means
although the type-I error level is allowed to be as large as $\alpha$,
the highest power in (\ref{eq:slope_test_opt_ubd}) can actually be
achieved at a type-I error level less than $\alpha$. Therefore, we
can enforce a more stringent type-I error level constraint, without
losing the power. In particular, let $\alpha':=\P(|\sigOpt H|\geq\ythresh)<\alpha$
and we can show $\overline{\mathcal{\limpower}}(\alpha')=\overline{\mathcal{\limpower}}(\alpha)$.
Indeed, on one hand, we have $\overline{\mathcal{\limpower}}(\alpha')\leq\overline{\mathcal{\limpower}}(\alpha)$,
since $\alpha'<\alpha$ and $\alpha\mapsto\overline{\mathcal{\limpower}}(\alpha)$
is non-decreasing; on the other hand, since $\P(|\sigOpt H|\geq\ythresh)=\alpha'$,
we obtain that $\mealim_{\text{opt},\alpha}$ is also a feasible solution
of (\ref{eq:slope_test_opt_ubd}) under the type-I error level $\alpha'$.
Also when $\mealim_{\Lambda}=\mealim_{\text{opt},\alpha}$, the objective
value of (\ref{eq:slope_test_opt_ubd}) equals to $\overline{\mathcal{\limpower}}(\alpha)$.
Therefore, we have $\overline{\mathcal{\limpower}}(\alpha')\geq\overline{\mathcal{\limpower}}(\alpha)$
and thus, $\overline{\mathcal{\limpower}}(\alpha')=\overline{\mathcal{\limpower}}(\alpha)$.
Meanwhile, 
\begin{align*}
\limpower(\alpha') & \geq\P(|B+\sigOpt H|\geq\ythresh\mid B\neq0)\\
 & =\P(|B+\sigOpt H|\geq\Phi^{-1}(1-\tfrac{\alpha'}{2})\sigOpt\mid B\neq0)\\
 & =\overline{\mathcal{\limpower}}(\alpha'),
\end{align*}
where the inequality follows from the fact that $\mealim_{\Lambda}=\mealim_{\text{opt},\alpha}$
is a feasible solution of (\ref{eq:slope_test_opt}) under type-I
error level $\alpha'$, the first equality is due to $\alpha'=\P(|\sigOpt H|\geq\ythresh)$
and the second equality follows from the fact that $\mealim_{\text{opt},\alpha}$
is an optimal solution of (\ref{eq:slope_test_opt_ubd}) under type-I
error level $\alpha'$ {[}recall that $\overline{\mathcal{\limpower}}(\alpha')=\overline{\mathcal{\limpower}}(\alpha)${]}.
Since $\overline{\mathcal{\limpower}}(\alpha')$ is also the upper
bound of $\limpower(\alpha')$, we then conclude that $\limpower(\alpha')=\overline{\mathcal{\limpower}}(\alpha')$.
Combining the above results together and using our assumption that
$\overline{\mathcal{\limpower}}(\alpha)>\limpower(\alpha)$, we have
\[
\limpower(\alpha')=\overline{\mathcal{\limpower}}(\alpha')=\overline{\mathcal{\limpower}}(\alpha)>\limpower(\alpha)\geq\limpower(\alpha'),
\]
which leads to a contradiction. Therefore, we prove that $\limpower(\alpha)=\overline{\mathcal{\limpower}}(\alpha)$.

Finally, since $\overline{\mathcal{\limpower}}(\alpha)$ and $\mealim_{\text{opt},\alpha}$
are the optimal value and solution of (\ref{eq:slope_test_opt_ubd}),
we know $\limpower(\alpha)=\overline{\mathcal{\limpower}}(\alpha)$,
when $\mealim_{\Lambda}=\mealim_{\text{opt},\alpha}$.

\begin{comment}
Also since $\delta^{-1}\E\big[\proxfree_{\alpha}'(\toptY)\big]<1$,
by Lemma \ref{lem:testing_tightness_cond_2}, we know the upper bound
(\ref{eq:powerubd}) can be attained when $\mealim_{\Lambda}=\mealim_{\text{opt},\alpha}$.
This concludes our proof.
\end{comment}
\end{IEEEproof}


